Single ion spectroscopy of four metastable state clear-out transitions in Yb II: isotope shifts and hyperfine structure

We present spectroscopic data for four metastable state clear-out transitions between 399 nm and 412 nm for all even long-lived isotopes of Yb$^+$ as well as their hyperfine structure in $^{171}$Yb$^+$. The strong $^2 \rm{D}_{3/2} \rightarrow {}^1[1/2]_{1/2}$ transition at 412 nm represents an attractive alternative for the standard 935 nm repumper used in cooling and trapping experiments, while the transition to the $^3[3/2]_{3/2}$ state at 411 nm clears out the $^2 $F$_{7/2}$ state, for which typically 638 nm or 760 nm are used. These two alternative transitions simplify the experimental setup by removing the need for infrared optics to cool and manipulate Yb$^+$ and may be of particular interest when considering integrated photonics solutions. We also present data for the transitions $^2 $D$_{3/2} \rightarrow {}^3[1/2]_{3/2}$ at 399 nm, and $^2 $D$_{3/2} \rightarrow {}^1[5/2]_{5/2}$ at 410 nm including decay branching ratios of the excited states.

==> oldtext.tex <==

\setlength{\tabcolsep}{10pt}
\begin{longtable}[c]{@{}cccc@{}}
\toprule \hline 
Isotope & 399 nm    & 935 nm     & 412 nm   \\* \midrule
\endfirsthead
%
\multicolumn{4}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\toprule
Isotope & 399 nm    & 935 nm     & 412 nm   \\* \midrule
\endhead
%
\bottomrule
\endfoot
%
\endlastfoot
%
168     & 751.52829 & 320.562142 & 727.533757(2) \\
170     & 751.52764 & 320.565872 & 727.537170(2) \\
171     & 751.52724 & 320.569242 & 
\\
172     & 751.52694 & 320.569352 & 727.540363(1)  \\
174     & 751.52643 & 320.571972 & 727.542755(3) \\
176     & 751.52592 & 320.574462 & 727.545028(3) \\  \hline \bottomrule

\caption{Frequencies in THz. Wavemeter error 8 MHz }
\label{tab:my-table}\\
\end{longtable}




 

%The 410 nm clear out transition couples $^2D_{3/2} \rightarrow ^1[5/2]_{5/2} $. From this state it can only decay to the $^2D_{5/2} $ state. To find the hyperfine splitting we do the following pulse scheme. The ion is doppler cooled with the 369 nm and 935 nm lasers. Then the ion is shelved in the $^2D_{3/2} $ state by given a 369 nm pulse. In a third step, this state is emptied by a 410 nm pulse if it is on resonance. It can then decay to the  $^2D_{5/2} $. We then wait for a time twait for the $^2D_{5/2} $  to decay. To state detect do a pulse of 369 nm and 935 nm. If the ion was not pumped out if appears bright. If it decayed to $^2F_{7/2}$, it appears dark. We scan over frequency and find three dips in fluoresence. One of the dips is separate by 860() MHz which we attribute to the hyperfine splitting of the $^2D_{3/2}$ state. The second splitting at  1414() MHz is then the splitting of the upper $^1[5/2]_{5/2}$ state. Since the $^2D_{3/2} $ F = 1 state can only couple to the $^1[5/2]_{5/2}$ F = 2 state and the we find the third peak of F = 2 $\rightarrow$ F’=3 at a higher frequency we see that the F’=3 is higher in frequency than the F’=2 in the $^1[5/2]_{5/2}$ state. 
%To  the $^1[5/2]_{5/2}$ can only decay to the the $^2D_{5/2} $ due to parity rules. The the $^2F_{7/2} $ has the parity (odd) as the $^1[5/2]_{5/2}$ state which means it is dipole forbidden. To check that nothing (bit stong word) decay to the $^2F_{7/2} $ state we do a branching ratio mearement. First the ion is shelved in the the $^2D_{5/2} $ state
%by given a 369 nm pulse. In a second step, this state is emptied by a 410 nm pulse. It then decays with a branching ratio b to the$^2D_{5/2} $ state. And a possible bracnching ratio of 1-b to $^2F_{7/2} $ We then wait for a time twait for the $^2D_{5/2} $to decay for …. ms. To state detect do a pulse of 369 nm and 935 nm. If the ion only decayed to the $^2D_{5/2} $ we find a 17~\% of it appearing bright, since this is just the branching ratio of the $^2D_{5/2} $ state \cite{}. If it also has an decay path to the $^2F_{7/2}$ state we expected a lower value than 17~\%/ We find the ion bright around 17()~\% of time indicating no direct decay to the $^2F_{7/2} $. As a test we vary the pulse length of the 410 nm laser to show we pump out the $^2D_{3/2} $ state completely. We find an asymtotoic value of 17~\% as the pulse length is increased. 

%The 411 nm drives the $^2F_{7/2} \rightarrow ^3[3/2]_{3/2} $ transition to re-repump back the ion. To measure the hyperfine splitting we do the following sequence. The ion is doppler cooled with the 369 nm and 935 nm lasers. Then the ion is shelved in the $^2F_{7/2} $ state by given a 369 nm pulse and 399 nm pulse which pumps it to the $^2D_{5/2} $ state from which it decays to the $^2F_{7/2} $ state. Since the branching ratio of the 399 nm is quite small to the $^2D_{5/2} $ state, we do a long pulse of …. ms with the 369 nm on as well to increase the probability to end up in the $^2F_{7/2} $ state Then a 411 nm pulse is given for … ms. After which we do state detection using the 369 nm and 935 nm laser. If the ion is bright, it was pumped back succesfully, otherwise it remains dark. Afterwards we pump the ion back the 760 nm and cool it again. We scan the frequency of the 411 nm and find 3 peaks in fluoresence. Two peaks are split by 3620() MHz which we attribute to the hyperfine splitting of the groundstate. The thrid peak is very close to one of the other peaks. Since the F=4 of the $^2F_{7/2} $ state can only couple to F’ = 2 of the  $^3[3/2]_{3/2} $ we know that the 

%We put the 399 nm to drive the F = 1 $^2D_{3/2}$ to F’=1 $^3[1/2]_{3/2} $ transition, meaning it can only decay to the F = 3 of the $^2F_{7/2}$ state. We then find two peaks in fluoresence with a splitting of 3645() MHz. We then drive the 399 nm on the F = 1 $^2D_{3/2}$ to F’=2 $^3[1/2]_{3/2} $ transtion which means it could end up in either the F = 3 or F=4 of the $^2F_{7/2}$ state. We find only 1 peak which it exactly the hyperfine spiltting of the groundstate of 3620()MHz \cite{} away from one of the other peaks we found earlier. Indicate the F = 4 $^2F_{7/2}$  $\rightarrow $ F’=2 $^3[3/2]_{3/2}$. We do not find other peaks indicating it might be very unlikely to end up in the F=3 $^2F_{7/2}$ state .

% To show this we also scan the 760 nm frequency and find that we almost nothing ends up in the F=3 state. We also scan the 760 nm to find the hyperfine splitting using the method described above but now using the 411 nm as a re-repump to get the ions back into the cooling cycle. We find three peaks in fluoresence. One of the spilling is 3620()~MHz as already measured before with the 411 and shown in other work \cite{}. The other spilitting of the upper state $^3[3/2]_{3/2}$ given by 8880()~MHz, already measured in \cite{} but improved precision with this worlk. 

\warn{might be nice to in the table to put for 171 either the CoM of the transition or put the frequency that we used for the hyperfine where the "0" is and then calculate the isotope shift from this? }

 %            & \text{$^2 D_{3/2} \rightarrow {}^3[3/2]_{1/2}$}  & \text{$^2 D_{3/2} \rightarrow {}^1[1/2]_{1/2}$}   & \text{$^2 D_{3/2} \rightarrow {}^3[1/2]_{3/2}$}    & \text{$^2 D_{3/2} \rightarrow {}^1[5/2]_{5/2}$}& \text{$^2 F_{7/2} \rightarrow {}^1[3/2]_{3/2}$}   & \text{$^2 F_{7/2} \rightarrow {}^1[3/2]_{3/2}$}   \\ \hline


\begin{table*}[t]
\centering
\begin{tabular}{cccccccc}
\hline
  Lower state           & \multicolumn{4}{c}{\text{$^2 D_{3/2}$}  } & & \multicolumn{2}{c}{\text{$^2 F_{7/2}$}   }    \\ 
  & & McC. & Len & Starr & &  &Harr\\
Upper state             & \text{${}^3[3/2]_{1/2}$}  & \text{${}^1[1/2]_{1/2}$}   & \text{${}^3[1/2]_{3/2}$}    & \text{${}^1[5/2]_{5/2}$}& & \text{${}^1[3/2]_{3/2}$}   & \text{$^1[3/2]_{3/2}$}   \\ \hline
Isotope             & 935 nm    & 412 nm    & 399 nm    & 410 nm & &760 nm    & 411 nm    \\ \hline
168                 & 320.56214 & 727.53376 & 751.39459 &        & &394.43287 & 729.06140 \\
170                 & 320.56587 & 727.53717 & 751.39589 &        & &394.42959 & 729.05694 \\
171                 & 320.56924 &           &           &        & &          &           \\
HF & 0.86 GHz  & 0.87 GHz  & 0.71 GHz  &        & &8.88 GHz   &   3.64 GHz        \\
172                 & 320.56935 & 727.54036 & 751.39711 &        & & 394.42655 & 729.05275 \\
174                 & 320.57197 & 727.54275 & 751.39796 &  & & 394.42415 & 729.04950 \\
176                 & 320.57446 & 727.54503 & 751.39877 &        & & 394.42189 & 729.04646 \\ \hline
\end{tabular}%
\caption{Frequencies in THz. Wavemeter error 8 MHz}
\label{tab:my-table}
\end{table*}



\begin{table*}[t]
\centering
\begin{tabular}{cccccccc}
\hline
  Lower state           & \multicolumn{4}{c}{\text{$^2 D_{3/2}$}  } & & \multicolumn{2}{c}{\text{$^2 F_{7/2}$}   }    \\ 
  & & McC. & Len & Starr & &  &Harr\\
Upper state             & \text{${}^3[3/2]_{1/2}$}  & \text{${}^1[1/2]_{1/2}$}   & \text{${}^3[1/2]_{3/2}$}    & \text{${}^1[5/2]_{5/2}$}& & \text{${}^1[3/2]_{3/2}$}   & \text{$^1[3/2]_{3/2}$}   \\ \hline
Isotope             & 935 nm    & 412 nm    & 399 nm    & 410 nm & &760 nm    & 411 nm    \\ \hline
168                 & 320.56214 & 727.53375744(21) & 751.3945936(7) & 730.54803307(14)       & &394.43287 & 729.0613977(12) \\
170                 & 320.56587 & 727.53717207(27) & 751.3958990(4) & 730.55073813(18) & &394.42959 & 729.0569416(5) \\
172                 & 320.56935 & 727.54036010(16) & 751.39711176(21) &  730.5532596(4)      & & 394.42655 & 729.05276991(32) \\
174                 & 320.57197 & 727.54275436(20) & 751.39785765(11) &  730.55513343(17) & & 394.42415 & 729.04953603(34) \\
176                 & 320.57446 & 727.54502848(26) & 751.39877853(12) & 730.55690796(21)     & & 394.42189 & 729.04645854(28) \\ \hline
\end{tabular}%
\caption{Frequencies in THz. All measurement errors and precision. All results taken from the }
\label{tab:my-table}
\end{table*}


\begin{table*}[t]
\centering
\begin{tabular}{cccccccc}
\hline
  Lower state           & \multicolumn{4}{c}{\text{$^2 D_{3/2}$}  } & & \multicolumn{2}{c}{\text{$^2 F_{7/2}$}   }    \\ 
  & & McC. & Len & Harr & &  &Starr\\
Upper state             & \text{${}^3[3/2]_{1/2}$}  & \text{${}^1[1/2]_{1/2}$}   & \text{${}^3[1/2]_{3/2}$}    & \text{${}^1[5/2]_{5/2}$}& & \text{${}^1[3/2]_{3/2}$}   & \text{$^1[3/2]_{3/2}$}   \\ \hline
Isotope             & 935 nm    & 412 nm    & 399 nm    & 410 nm & &760 nm    & 411 nm    \\ \hline
168                 & -7210 & -6600 & -2520 &        & & 6320 & 8650 \\
170                 & -3480 & -3190 & -1220 &        & & 3040 & 4190\\
171                 &  &           &           &        & &          &           \\
HF & 0.86 GHz  & 0.87 GHz  & 0.71 GHz  &        & &8.88 GHz   &   3.64 GHz        \\
172                 & 0 & 0 & 0 &        & & 0 & 0 \\
174                 & 2620  & 2390 & 580 &        & & -2400 & -3250\\
176                 & 5110 & 4670 & 1660 &        & & -4660 & -6290 \\ \hline
\end{tabular}%
\caption{Isotope shifts in MHz. Wavemeter error 8 MHz \warn{the 410 transition is measure, just has to be put in here}}
\label{tab:my-table}
\end{table*}


\begin{table*}[t]
\centering
\begin{tabular}{llllllllllll}
\hline
\multicolumn{2}{c}{935\,nm } &\phantom{d} & \multicolumn{2}{c}{760\,nm }&\phantom{d} & \multicolumn{2}{c}{411\,nm }  \\
\multicolumn{2}{c}{${}^2\text{D}_{3/2}\rightarrow{}^3\text{[3/2]}_{1/2}$} &\phantom{d} & \multicolumn{2}{c}{${}^2\text{F}_{7/2}\rightarrow{}^1\text{[3/2]}_{3/2}$}&\phantom{d} & \multicolumn{2}{c}{${}^2\text{F}_{7/2}\rightarrow{}^3\text{[3/2]}_{3/2}$}  \\
  \hline
F=2 $\rightarrow$ F=1& 320.5661765(9)& &F=3 $\rightarrow$ F=1 & 394.4249689(6) & &F=4$\rightarrow$ F=2 & 729.0552436(8)\\
F=1 $\rightarrow$ F=1 &  320.5670353(8) & &F=3 $\rightarrow$ F=2 & 394.4338479(7) & &F=3$\rightarrow$ F=1 & 729.0552103(6) \\
F=1 $\rightarrow$ F=1 & 320.56924432(33)& &F=4 $\rightarrow$ F=2 & 394.4302248(7) & &F=3$\rightarrow$ F=2& 729.0588572(16)\\
 \hline
\end{tabular}%
\caption{935 F=2 $\rightarrow$ F=1: Folder06, the other two from their respective folder 04.}
\label{tab:my-table}
\end{table*}

